Large sets containing no copies of a given infinite sequence

Suppose $a_n$ is a real, nonnegative sequence that does not increase exponentially. For any $p<1$ we contruct a Lebesgue measurable set $E \subseteq \mathbb{R}$ which has measure at least $p$ in any unit interval and which contains no affine copy $\{x+ta_n:\ n\in\mathbb{N}\}$ of the given sequence (for any $x \in \mathbb{R}, t > 0$). We generalize this to higher dimensions and also for some ``non-linear'' copies of the sequence. Our method is probabilistic.

==> avoid-1.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-1_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-387.208418,9.733105)(-0.500000,-1.000000){-4}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-341.684008,9.733105)(-0.500000,-0.969390){-3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-296.159599,9.733105)(-0.500000,-1.000000){-2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-250.635189,9.733105)(-0.500000,-1.000000){-1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-205.110780,9.733105)(-0.500000,-0.969390){0}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-159.586371,9.733105)(-0.500000,-1.000000){1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-114.061961,9.733105)(-0.500000,-1.000000){2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-68.537552,9.733105)(-0.500000,-0.969390){3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-23.013142,9.733105)(-0.500000,-1.000000){4}%


==> avoid-2.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-2_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-319.089754,11.501115)(-0.500000,-0.820001){$-N_n \cdots$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-292.666233,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-266.242712,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-239.819190,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-213.395669,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-186.972148,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-160.548627,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-134.125106,11.501115)(-0.500000,-1.000000){.}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-107.701585,11.501115)(-0.500000,-0.820001){$\cdots N_n$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-213.395669,10.179939)(-0.500000,-1.000000){$0$}%


==> avoid-3.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-3_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-387.208418,10.701125)(-0.500000,-0.891304){$-N \cdots$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-341.684008,10.701125)(-0.500000,-0.969390){-3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-296.159599,10.701125)(-0.500000,-1.000000){-2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-250.635189,10.701125)(-0.500000,-1.000000){-1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-205.110780,10.701125)(-0.500000,-0.969390){0}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-159.586371,10.701125)(-0.500000,-1.000000){1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-114.061961,10.701125)(-0.500000,-1.000000){2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-68.537552,10.701125)(-0.500000,-0.969390){3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-23.013142,10.701125)(-0.500000,-1.000000){$\cdots N$}%


==> avoid-4.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-4_0}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-387.208418,10.701125)(-0.500000,-0.891304){$-N \cdots$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-341.684008,10.701125)(-0.500000,-0.969390){-3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-296.159599,10.701125)(-0.500000,-1.000000){-2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-250.635189,10.701125)(-0.500000,-1.000000){-1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-205.110780,10.701125)(-0.500000,-0.969390){0}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-159.586371,10.701125)(-0.500000,-1.000000){1}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-114.061961,10.701125)(-0.500000,-1.000000){2}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-68.537552,10.701125)(-0.500000,-0.969390){3}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-23.013142,10.701125)(-0.500000,-1.000000){$\cdots N$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-306.292585,19.122930)(-1.000000,0.000000){$x$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-159.586371,40.663330)(-0.500000,0.282848){$x+t_1a_{n_1}$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-159.586371,86.187739)(-0.500000,0.282848){$x+t_2a_{n_2}$}%


==> avoid-5.tex <==
\setlength{\unitlength}{1pt}%
\makeatletter%
\let\ASYencoding\f@encoding%
\let\ASYfamily\f@family%
\let\ASYseries\f@series%
\let\ASYshape\f@shape%
\makeatother%
{\catcode`"=12%
\includegraphics{\ASYprefix\jobname-5_0}%
}%
\special{pdf:literal q}%
\begin{picture}( 284.527559, 227.622047)%
\special{pdf:literal \ASYraw{
 -283.464567 0.000000 m
 0.000000 0.000000 l
 0.000000 226.771654 l
 -283.464567 226.771654 l
 -283.464567 0.000000 l
h
W n
}%
}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\usefont{\ASYencoding}{\ASYfamily}{\ASYseries}{\ASYshape}%
\ASYalign(-142.263780,88.958268)(-0.500000,0.179999){$T_1$}%
\definecolor{ASYcolor}{gray}{0.000000}\color{ASYcolor}%
\fontsize{12.000000}{14.400000}\selectfont%
\ASYalign(-71.131890,69.041339)(-0.500000,0.179999){$T_2$}%
\end{picture}%
\kern -284.527559pt%
\special{pdf:literal Q}%

